A rigorous path integral for quantum spin using flat-space Wiener regularization

Adapting ideas of Daubechies and Klauder [J. Math. Phys. {\bf 26} (1985) 2239] we derive a rigorous continuum path-integral formula for the semigroup generated by a spin Hamiltonian. More precisely, we use spin-coherent vectors parametrized by complex numbers to relate the coherent representation of this semigroup to a suitable Schr\"odinger semigroup on the Hilbert space $L^2(R^2)$ of Lebesgue square-integrable functions on the Euclidean plane $R^2$. The path-integral formula emerges from the standard Feynman-Kac-It\^o formula for the Schr\"odinger semigroup in the ultra-diffusive limit of the underlying Brownian bridge on $R^2$. In a similar vein, a path-integral formula can be constructed for the coherent representation of the unitary time evolution generated by the spin Hamiltonian.

==> definitionen.tex <==
\RequirePackage{amsbsy}

%
%e-Funktion
\newcommand\ep[1]{{e}^{\,\mbox{\small $ #1 $}}}
%
%one (unity)
\newcommand\one{\leavevmode\hbox{\small1\kern-3.78pt\normalsize1}}%
%1/2
\newcommand\half{{\frac 12}}

%Wiener
\newcommand{\dmut}{\int  \mkern-6mu d \mu_{z\!,0;z',t}^{(\nu)}(b) \;}
\newcommand{\dmuu}{\int  \mkern-6mu d \mu_{z\!,0;z',u}^{(\nu)}(b) \;}
\newcommand{\Idmut}{d \mu_{z\!,0;z',t}^{(\nu)}(b)}

% Command for Bras. Example: with "\bra{1}" you get "<1|".
\newcommand{\ket}[1]{|\mkern0.2mu\mbox{$#1$}\rangle}  
% \ket{1}: |1>
\newcommand{\bra}[1]{\langle\mbox{$#1$}\mkern0.2mu|}              
\newcommand\braket[2]{\langle#1|#2\rangle}
%
%Dickerpunkt
\newcommand\bcdot{\mbox{\boldmath$\cdot$\unboldmath}}
%
\newcommand\abs[1]{\left\vert {#1}\right\vert}
%
\newcommand{\eq}[1]{(\ref{#1})}
%
\newcommand\norm[1]{{\left\vert\mkern-2mu\left\vert #1 \right\vert\mkern-2mu\right\vert}}
%
\renewcommand{\labelenumi}{(\roman{enumi})}
